Revisiting Few-shot Relation Classification: Evaluation Data and Classification Schemes

We explore Few-Shot Learning (FSL) for Relation Classification (RC). Focusing on the realistic scenario of FSL, in which a test instance might not belong to any of the target categories (none-of-the-above, aka NOTA), we first revisit the recent popular dataset structure for FSL, pointing out its unrealistic data distribution. To remedy this, we propose a novel methodology for deriving more realistic few-shot test data from available datasets for supervised RC, and apply it to the TACRED dataset. This yields a new challenging benchmark for FSL RC, on which state of the art models show poor performance. Next, we analyze classification schemes within the popular embedding-based nearest-neighbor approach for FSL, with respect to constraints they impose on the embedding space. Triggered by this analysis we propose a novel classification scheme, in which the NOTA category is represented as learned vectors, shown empirically to be an appealing option for FSL.

==> exhaustive_evaluation.tex <==
\ol{
\subsection{Exhaustive 1-Way 1-Shot Evaluation}


The optimal evaluation for the \nwks{} setting is to exhaustively compare every K instances for each N relations. As this is an exponential space, it is not feasible to compute in practice. Therefore, the standard evaluation method is to sample episodes and to report the average score based on these sampling (as discussed in Sec \ref{TASK_SETUP}). 
We propose here an exhaustive evaluation for the 1-Way 1-Shot setting, where we provide a fast and accurate evaluation for this setting, accounting for Precision, Recall and F1.

% In the common \nwks{} setting, a model is evaluated based on its performance on a sequence of episodes. As episodes are generated randomly, performances may vary greatly between sequences of episode. To overcome this randomization noise, we evaluate on large number of episodes. This evaluation practice requires much resources and long time. We suggest a method to directly compute the f1, recall, and precision, in 1-way 1-shot experiments.
To this end, we compute the False Positive Rate (FPR) and False Negative Rate (FNR) per instance, which is then averaged across all instances to get the overall precision and recall. 

Let $R_i$ be the set of instances which correspond to class $c_i$, and let $M_i$ be the set of all other instances (instances which do not correspond to class $c_i$). 

To compute the FPR of instance $r \in R_i$, we define an indicator function which gets as input another instance and outputs $1$ if the similarity between them is larger than the NOTA score.
As this evaluation process is agnostic to the method we use to compute the NOTA category score, we denote it by $S_N$ regardless if the score is obtained by similarity between $r_i$ and the NAV or by a fixed-threshold.
This function is formally defined as:
% We define an indicator function that gets as input an instance, and output 1 if 
\begin{equation*}
\mathbf{1}_{x_r}(x_m) :=
\begin{cases}
1 &\text{if } sim(x_r,x_m) > S_{N}, \\
0 &\text{ Otherwise }
\end{cases}
\end{equation*}
With this function we count how many single instance \sups{} yields false positive classifications. Let $r$ be the test query, we sum over all instance (\sups{} of size one) from distinct classes to compute the instance FPR.    
Formally, we compute the instance FPR as follows: 
 % could also be written in an expect form

\begin{equation*}
   \text{FPR}_{\mathbf{x_r}} = \frac{\sum\limits_{x_m \in M_i} \mathbf{1}_{x_r}(x_m) }{|M_i|}
\end{equation*}




In analogy but opposite manner, we compute the instance FNR by summing the indicator function over all instances in the same class, $R_i$:
\begin{equation*}
  \text{FNR}_{\mathbf{x_r}} = \frac{\sum\limits_{x_m \in R_i} (1 - \mathbf{1}_{x_r}(x_m)) }{|R_i|}
\end{equation*}

Finally, to compute the precision and recall micro score we average all instances FPR and FNR, respectively. Similarly, we can compute the macro level scores, by averaging across in class level.
}

==> named_entities_experiment.tex <==
\begin{figure}[]
\centering
\includegraphics[width=7cm,height=3.5cm]{images/Named Entities vs All Entity Forms.png}
\caption{\os{F1 scores on two subsets of relation instances. The relation instances are divided into two categories. Blue: Both target entities are named entities. Red: One of the target entities is a pronoun or a common noun. Results on \fstac{} for the 1-shot, and 5-shot settings}}
\label{fig:common_noun_vs_named_entities}
\vspace{-.5cm}
\end{figure}


% \begin{figure}[!t]
% \centering
% \includegraphics[width=7cm]{images/controlled_Named Entities v. Common Nouns.png}
% \caption{\os{F1 scores on two subsets of relation instances. The relation test instances are divided into two categories. Blue: Both target entities are named entities. Red: One of the target entities is a pronoun or a common noun. The three leftmost columns are evaluated on our new \fstac{} test set while the rightmost belongs to TACRED dataset. Results on \fstac{} for the 1-shot, and 5-shot settings, along with the results of a supervised model evaluated against the same test set. For TACRED dataset we trained a supervised model.}}
% \label{fig:common_noun_vs_named_entities}
% % \vspace{.5cm}
% \end{figure}

==> old_background.tex <==
\section{Related Work}
\label{Related_Work}
\ol{
\begin{itemize}
    % \item \nwks~as the standard evaluation for FSL.  this is in the task
   \item 2.1 Few Shot RE Datasets - high level
   \item !! focus on RE few shot space, relate to prior generic ML work on few shot
   \begin{itemize}
       \item FewRel - mention episodes, ML roots
       \item FewRel 2. Mention this is the setting we follow.
       \item Add: note on the synthetic distribution in FewRel, vs. the "natural/realistic" category distribution in supervised RE datasets. Forward reference to our contribution over TACRED
   \end{itemize}
   \item Modeling
   \begin{itemize}
       \item Embedding learning - MTB, as FewRel SOTA,  with its roots in Snell and other works. (merge the two corresponding paragraphs)
       \item FewRel 2 baseline - merge into here the BERT sentence pair paragraph in 5
       \item say we focus on embedding learning and similarity, and motivate - advantages, weaknesses of BERT pair approach.
       \item mention FSL extensions in generic ML beyond the embedding + nearest neighbor - further utilization of the support set - 1-2 sentences, these may interesting extensions to combine with our models.
   \end{itemize}
\end{itemize}
   
   
%     \item Common approaches for FSL
%     \item Both the approaches used the transfer learning approach which utilize a distinct labeled data source  
%     \begin{itemize}
%         \item Embedding learning SNELL et al and more
%             \item Skim previous works in NLP, go over this work
%             \item add a sentence or so from the works Yanai has sent, maybe by cluster of methods
%         \item Model-agnostic Meta-learning FINN et al
%             \item A Few-Shot work in NLP, text classification -  https://openreview.net/pdf?id=H1emfT4twB
%         % \item Data augmentation - as a orthogonal approach
%     \end{itemize} 
%     % \item Few-shot with OOD does not have enough work -> move into introduction, when you mention that there were few OOD in FSL works
%     % \item FSL with OOD, a work which was rejected from ICLR - https://openreview.net/pdf?id=BygNAa4YPH
%     % \item FewRel 2 as the first Few-shot OOD task. 
%     \item RE - many previous work. A lot of work on supervised RE
%     \item few different datasets, we focus on TACRED and propose transformation method from supervised dataset into FSL dataset. cite MTB in this paragraph as another work on RE 
%     \item Few-Shot RE previous works: 
%     \item First work to path the way for better FSL in RE: dataset 
%     \begin{itemize}
%         % \item a more challenging task
%         \item MALAM and other Previous work (not including MTB) 
%         \item MTB work: embedding function, SOTA on multiple datasets
%         % \item works on distant supervision
%     \end{itemize}
%     \item Zero shot learning - a work by Omer Levy? to introduction
%     % \item \nwks~with NOTA extension in FewRel2
% \end{itemize}

}
% \paragraph{Common Few-Shot learning approaches.}
% Lately, Few-Shot Learning (FSL) gained a lot of attention in the Machine Learning community. 
% Methods that tackle the FSL setup can be roughly divided into two main methods: \textit{Embedding Learning} and \textit{Optimization-Based}.

% Few-Shot Learning (FSL) has recently gained much interest.

\paragraph{Few-Shot Relation Extraction datasets.}

Recently, the first dedicated Few-Shot Learning Relation Extraction (RE) dataset - FewRel was released \cite{FEWREL}. It consists of $100$ relation types, each contains $700$ relation instances, which were spilt into $64$, $16$, and $20$ categories in the train, dev and test sets, respectively. Overall there are $70,000$ labeled relation instances in FewRel which makes it the largest RE dataset to date. 
FewRel relation instances were collected based on Wikipedia and labeled using Wikidata. Human annotators verified the correctness of the sentence labels. 
The fact that all relation classes possess the same number of instances, regardless to any truthful distribution in a corpus, manifest this dataset as a synthetic one. As opposed, supervised RE datasets such as, TACRED and DocRED \cite{tacredzhang2017,DocRED} were collected with respect to the relation distribution in an existing corpus. In Section \ref{TRANSFORMATION}, we propose a methodology to transform any supervised dataset into FSL dataset while maintaining the dataset category distribution. 

In addition to the dataset itself, FewRel work also suggests to adapt the common \nwks{} setting for Few-Shot Learning (FSL) \cite{snell2017prototypical,vinyals2016matching,maml_finn,ravi2016optimization}. 
In a follow up work, FewRel2 \cite{FEWREL_second}, introduces a more challenging setting based on the FewRel dataset, which we detail in Section \ref{TASK_SETUP}. 
% In this work, the setup is identical to the original setup, but an additional option is introduced at test-time: NOTA, where none of the given relations match the query. The authors introduced a modification to the original dataset where the NOTA option is part of the classification options.


% and can roughly be divided into two main methods: \textit{Embedding Learning} and \textit{Optimization-Based}. Both approach origins are founded at the transfer learning approach which assumes the existing of a labeled dataset for a distinct task. 


% In this work we focus on the Embedding Learning modeling scheme, in which instances are embedded into a vector space. In this scheme, instances of the same class should be embedded close, while instances from distinct classes should be embedded further apart. To classify a test instance one 






% In Embedding Learning, instances are embedded into a vector space, in which instances of the same label should be embedded close, while instances from distinct labels should be embedded further apart \cite{koch2015siamese,vinyals2016matching,learning_to_compare,DBLP:journals/corr/MehrotraD17}. In the noteworthy prototypical network work, \citet{snell2017prototypical} proposed to represent a class by averaging all its embedded labeled instances into a single vector in the vector space, called \textit{prototype}. Then, at test time, instances are classified according to their nearest prototype. Recently several works adapted the prototypical approach for FSL applied on text classification \cite{prototypical_in_text_classification,prototypical_text_clasification}.

% A new line of meta-learners for one-shot learning is rising lately: Ravi & Larochelle (2016) in- troduced a meta-learning method where an LSTM updates the weights of a classifier for a given episode. Munkhdalai & Yu (2017) also presented a meta-learning architecture that learns meta-level knowledge across tasks, and it changes its inductive bias via fast parametrization. Finn et al. (2017) is using a model agnostic meta-learner based on gradient descent, the goal is to train a classification model such that given a new task, a small amount of gradient steps with few data will be enough to generalize. Lately, Mishra et al. (2017) used Temporal Convolutions which are deep recurrent networks based on dilated convolutions, this method also exploits contextual information from the subset T providing very good results.

% A different perspective to tackle FSL is by treating it is as a \textit{meta-learning} problem (also known as \textit{Learning to Learn}). 
% \citet{ravi2016optimization} introduced the Optimization-Based line of research, which treats the FSL task as a \textit{meta-learning} problem (also known as \textit{Learning to Learn}). In these methods we learn good initialization parameters based on learning from multiple tasks, as such theses optimization methods are capable of solving a new learning task based only on few examples. 

% \textit{Optimization-Based} method for FSL \cite{ravi2016optimization}, treats it as a \textit{meta-learning} problem (also know as \textit{Learning to Learn}). In this approach, the goal is to learn an adaptive set of parameters that will generalize quickly to new examples. This is usually done by learning from multiple tasks.
% In \cite{maml_finn}, the authors suggested a framework for learning a set of parameters which is broadly applicable to a wide range of tasks. Their framework is agnostic to the model type and can be applied to all models that use gradient descent, including classification, regression, and reinforcement learning. 
% \ye{how is it different from the previous paragraph? If this work is important you should elaborate more on it, as right now it just looks the same}
% A notable work in this line of research is the Model-Agnostic Meta-learning \cite{maml_finn}, in which the authors suggest a method for learning a set of parameters which is broadly applicable to a wide range of tasks. 
% This approach differs from the classic supervised learning that aims to learn a task-specific set of parameters. 
% To satisfy this objective they minimize the total loss across distinct tasks. 
% \cite{ravi2016optimization,DBLP:conf/icml/MunkhdalaiY17}
% Another work in this category is \cite{ravi2016optimization}.

% An orthogonal method for addressing FSL is \textit{Data Augmentation}, in which more labeled instances are generated, as a result models can generalize better \cite{data_augmenation}. There are handful ways to perform this augmentation such as \textit{``handcrafted rules``}, for example e.g. converting the phrase \textit{``There's$\,\to\,$There is``}, or a \textit{``Learned Transformation``}, in which a function preforms a transformation on each training instance to generate more instances of the same label. 
% \textit{``bootstrapping``}, ??.
% These methods are generally useful and can be used on any model to improve its performance. In this work, we do not employ data augmentation, but note that theses methods can potentially improve the models performance. We leave the incorporation of these methods to future work.

% \paragraph{Relation Extraction prior works.} Relation Extraction (RE) is a well-known and a fundamental task in Information Extraction. RE allows to extract relation facts between entities from natural language text, that can be later used for various tasks such as question answering \cite{RE_for_QA} and fact checking \cite{RE_for_fact_checking}.
% % Few RE resources were released \cite{tacredzhang2017,DocRED}. 
% \ye{note: just a thought, but maybe the details about tacred and fewrel should be moved to another section.}
% In this work, we utilize the popular \textit{TACRED} RE dataset \cite{tacredzhang2017}, which contains 106,264 examples, built over newswire and web texts.
% % from the corpus used in the yearly TAC KB Population \footnote{\url{https://tac.nist.gov//2014/KBP/}} 
% Overall the dataset consists of 41 pre-defined relations, and an extra "no\_relation" class, which reflects all other relation types. 
% % TACRED relation instances were collected exhaustively on particular entities, thus the category distribution represents well the open information distribution \os{rephrase}. 
% TACRED was built in an exhaustive manner, such that the relations it contains represent their real distribution in texts.
% These datasets enable great progress in developing and publishing RE works  \cite{RE_first_work,DBLP:conf/emnlp/ZengLC015,MTB}. 

% In this work, we suggest a methodology to transform a supervised dataset into FSL dataset which we apply on TACRED. 






% \ye{add some discussion about FS for RE (don't start away with the dataset)}

% Recently, the first dedicated FSL RE dataset was released by \citet{FEWREL} (FewRel). It consists of 100 relations, which were spilt into 64,16,20 in the train, dev and test sets, respectively, each relation type consists of 700 relation instances. The relation instances were collected and labeled based on Wikipedia and Wikidata, then human annotators verified these labels. This dataset is the largest RE dataset to date.


% A recent work \cite{fewshot_text_classification_bao2020} has shown that common computer vision Meta-Learning methods applied directly on Natural Language Processing tasks, tend to perform poorly in various classification tasks. They proposed a new technique to learn the connection between word importance and distributional signatures which yields better performance. 

% Most prior work on weakly supervised RE was dedicated to leveraging information stored in knowledge bases (KB). \citet{Mintz_distant} proposed a distant supervision method to automatically align KB with text to get label training instances. Although distant supervision is an effective way to enlarge the training data, it inherently suffers from noisy data. Moreover, this approach mostly enriches dataset with the same common relations, hence the "long-tailed" relations still suffer from a lack of data.
% A recent work \citet{Noisy_RE} proposed handling this noisy labeled data, through attention mechanism on the support set. 
% In a parallel manner, \citet{Omer_levy} proposed a zero-shot RE method, by using a reading comprehension model. 
% Recently, \citet{FEWREL} have released the first dedicated dataset for Few-Shot relation extraction (FewRel). There are 64,16,20 relation types in the train, dev and test sets, respectively. Each relation type consists of 700 relation statements which were extracted from Wikipedia. They used Wikidata as relation label source and later annotators verified the relation depicts in the sentence. FewRel is the largest public RE dataset.
% FewRel2 \cite{FEWREL_second} is a follow up work that aims to tackle the unrealistic scenario that was introduced in FewRel. In this work, the setup is identical to the original setup, but an additional option is introduced at test-time: NOTA, where none of the given relations match the query. The authors introduced a modification to the original dataset where the NOTA option is part of the classification options.

% Further, they proposed a new baseline model which does not fall into one of the common FSL methods mentioned above. The suggested model leverages the next sentence prediction which BERT incorporates \cite{BERT}. Although, they get reasonably well results, their approach is memory inefficient and slow as they double each sentence length before feeding it to BERT. Further, concatenating two long sentences may exceed the BERT maximal length input, which make this model impossible to use for relatively long sentences.       



% In practice, this model which make this model impossible to use for relatively long sentences.      

% This architecture is depicted in Figure \ref{fig:1}. 

% The above process defines the MTB embedding function, in our work we would extend it to the new $N$-way $K$-shot with NOTA setup. 


% \begin{figure}[h]
% \centering
% \includegraphics[width=5cm]{MTB}
% \caption{Matching The Blanks final architecture}
% \label{fig:1}
% \end{figure}




% \paragraph{Few Shots Task}
% \label{background:few-shot-task}
% In this work, we are interested in the few-shot setting task \cite{few-shot work}. In this setting, we wish to to infer on new classes which were not seen during training, by solely a few examples. 
% Although this setting is harder than the usual supervised training, achieving good performance on this setting will remove \ye{wording} our need from massive amounts of data.
%In the simplest task variation the model has to classify an example from the new set of possible labels. As in many cases, there are a lot of different classes, which may not be present in the given set, we wish to be able to say that none of the new classes suit. This scenario is referred to as None-of-the-above (NOTA) \cite{first-work that did nota}.


% \paragraph{N-Way K-Shot Setting}
% A recently proposed evaluation setting is N-Way K-shot \cite{vinyals2016matching,@@}. In this setting, a model is presented with N classes, where each class consists of K examples.\footnote{Notice that this is a private case of a classification setting, where the number of examples per class is constant.} Each K examples from the same class in the evaluation examples are referred as the \textit{Support Set} \cite{snell2017prototypical}.\footnote{We keep the notations introduced by \citep{snell2017prototypical} rather then those defined in \citep{FEWREL} which define the Support set as the all of the examples from the entire data}.

% This setting gained popularity recently mainly in the few-shot scenario as it fits when K is small.
% Although the N-Way K-Shot setup is not restricted to the Few-Shot setup, in practice these are used the same, and in the rest of the paper when referring to n-way k-shot we also mean few-shot \ye{rephrase}.
% \ye{maybe add the nota also here as it doesn't get any examples}

% \paragraph{Few Shot Learning Schemes}
% As supervised methods require a lot of training data in order to generalize, training on the \nwks approach is probable to overfit.
% Thus, researchers have proposed different setups in order to overcome this problem.

% A common approach to deal with the few training examples is to perform the classification based on nearest-neighbors \cite{metric_learning,DBLP:conf/cvpr/LiWXHGL19}. In practice, the popular approach is to embed every instance using an embedding function and then use a similarity metric to determine the closest class. In this work, we follow the same approach.

% Given an instance from a new class, and the Support Set, we wish to measure similarity from the instance to the Support Set. \citet{snell2017prototypical} proposed to use a combination of the Support Set as its representative, which they define as the class's prototypical. In practice, they compute the prototypical of the Support Set as its mean.
% \citet{pmlr-v48-santoro16} proposed an alternative method, in which an RNN is trained to learn how to store and retrieve memories to use for each classification task.

% Multiple training methods for \nwks have been proposed like @@\cite{} and @@\cite{}. The current dominant approach is to have a similar training setup as the evaluation. This means that also during training, the model gets as input a \sups and a query and tries to maximize the similarity between the \sups and the correct class.
